Multi-turn Consistent Image Editing

Many real-world applications, such as interactive photo retouching, artistic content creation, and product design, require flexible and iterative image editing. However, existing image editing methods primarily focus on achieving the desired modifications in a single step, which often struggles with ambiguous user intent, complex transformations, or the need for progressive refinements. As a result, these methods frequently produce inconsistent outcomes or fail to meet user expectations. To address these challenges, we propose a multi-turn image editing framework that enables users to iteratively refine their edits, progressively achieving more satisfactory results. Our approach leverages flow matching for accurate image inversion and a dual-objective Linear Quadratic Regulators (LQR) for stable sampling, effectively mitigating error accumulation. Additionally, by analyzing the layer-wise roles of transformers, we introduce a adaptive attention highlighting method that enhances editability while preserving multi-turn coherence. Extensive experiments demonstrate that our framework significantly improves edit success rates and visual fidelity compared to existing methods.

==> algorithm/attention_mask.tex <==
\begin{algorithm}[htbp]
\caption{Medium-Low Activated Attention Mask Generation}
\label{alg:mask_generation}
\begin{algorithmic}[1]
\Require Query matrix \(Q\), key matrix \(K\), dimension \(d\), sampling step \(k\), threshold parameters: \(\text{threshold}\), \(\text{highlight\_factor}\), \(\text{reduce\_factor}\), and total number of double blocks \(N = 19\).
\Ensure Mask \(M_k\) guiding the image sampling process.
\For{each double block \(i = 1,2,\dots, N\)}
    \State Compute the attention map:
    \[
    s_{ki} \gets \operatorname{softmax}\Biggl(\frac{Q \cdot K^T}{\sqrt{d}}\Biggr)
    \]
    \State Binarize the attention map:
    \[
    s_{ki}^{\prime} \gets \sigma\Bigl(10\Bigl(\operatorname{normalize}(s_{ki}) - 0.5\Bigr)\Bigr)
    \]
\EndFor
\State Let \( S_k^{\prime} = \{s_{k1}^{\prime}, s_{k2}^{\prime}, \dots, s_{kN}^{\prime}\} \) be the set of attention maps sorted in ascending order based on activation intensity.
\State Select indices \(i\) and \(j\) (with \(1 \leq i < j \leq N\)) corresponding to the desired range of medium-low activations.
\State Define the subset of selected attention maps:
\[
S_{i,j} \gets \{ s_w \mid w \in \{i, i+1, \dots, j\} \}
\]
\State Compute the average activation of the selected maps:
\[
\bar{v}_{i,j} \gets \frac{\displaystyle\sum_{w=i}^{j} \sum\bigl(s_w\bigr)}{j - i + 1}
\]
\If{\(\bar{v}_{i,j} \geq \text{threshold}\)}
    \State Set \(M_k \gets \text{highlight\_factor}\)
\Else
    \State Set \(M_k \gets \text{reduce\_factor}\)
\EndIf
\State \Return \(M_k\)
\end{algorithmic}
\end{algorithm}

==> figures/midpoint.tex <==

\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{images/midpoint.pdf}
   \caption{Illustration of the standard midpoint method, a second-order ODE solver, that have better accuracy in single-step simutation ablity in discrete flow model.}
   \label{fig:midpoint}
\end{figure}

==> figures/multi_turn_reconstruct_double.tex <==
\newcommand{\downarrowwithtextleft}[2][OliveGreen, very thick]{
    \begin{tikzpicture}[baseline=(current bounding box.center)]
       
        \draw[->, line width=1pt, draw=#1, >=Latex] (0, 0) -- (0, -2); 
        
        \node[below=2pt, align=center, text=#1] at (0, -2) {#2}; 
    \end{tikzpicture}
}

\begin{figure*}[htbp]
    \centering
    \setlength{\tabcolsep}{2pt} 
    \renewcommand{\arraystretch}{0.8}

\hspace{-1.2cm}
\begin{tabular}{ p{1cm}@{\hspace{6pt}}c@{\hspace{18pt}}c}

    \begin{minipage}[t]{0.08\textwidth}
        \centering
        %\hspace{-1.3cm} % 调整箭头与子图之间的垂直间距
        \downarrowwithtextleft[OliveGreen, ultra thick]{\textit{Rec.} }
    \end{minipage}%

    &
  
    % 右侧区域：四行八列子图
    \begin{minipage}[t]{0.42\textwidth}
        \begin{tabular}{p{0.2cm}ccccc}
        \centering
        
            % 第0行
            & Ours & RF-Inv. & RF-Solv. & FireFlow & DDIM \\

             \vspace{-0.7cm}\textcolor{BrickRed}{\textit{0}} & \includegraphics[width=0.18\textwidth]{images/reconstruction/spiderman.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/spiderman.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/spiderman.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/spiderman.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/spiderman.jpg} \\

            % 第1行
            \vspace{-0.7cm}\textcolor{BrickRed}{\textit{1}} & 
            \includegraphics[width=0.18\textwidth]{images/reconstruction/mtf_r1.png} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Inversion_r1.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Solver_r1.png} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_spiderman_r1.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/ddim_spiderman_round1.jpg} \\

            
            % 第二行----------------------
            \vspace{-0.7cm}\textcolor{BrickRed}{\textit{2}} & \includegraphics[width=0.18\textwidth]{images/reconstruction/mtf_r2.png} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Inversion_r2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Solver_r2_2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_spiderman_r2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/ddim_spiderman_round2.jpg}  \\
            
            % 第三行----------------------
            \vspace{-0.7cm}\textcolor{BrickRed}{\textit{4}} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/mtf_r4.png} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Inversion_r4.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Solver_r4_2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_spiderman_r4.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/ddim_spiderman_round4.jpg} \\
            
            % 第四行----------------------
            \vspace{-0.7cm}\textcolor{BrickRed}{\textit{8}} &
           \includegraphics[width=0.18\textwidth]{images/reconstruction/mtf_r9.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Inversion_r8.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/RF-Solver_r8_2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_spiderman_r8.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/round8.jpg} 
        \end{tabular}
    \end{minipage}

    &

    \begin{minipage}[t]{0.42\textwidth}
        \begin{tabular}{ccccc}
            % 第一行
            Ours & RF-Inv. & RF-Solv. & FireFlow & DDIM \\

             \includegraphics[width=0.18\textwidth]{images/reconstruction/000000000011.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/000000000011.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/000000000011.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/000000000011.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/000000000011.jpg} \\
            
            
            \includegraphics[width=0.18\textwidth]{images/reconstruction/mtf__r1_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-inversion__r1_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-solver_r1_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_r2_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/ddim_bird_round1.jpg} \\

            
            % 第二行----------------------
            \includegraphics[width=0.18\textwidth]{images/reconstruction/mtf__r2_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-inversion__r2_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-solver__r2_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_r3_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/ddim_bird_round2.jpg} \\
            
            % 第三行----------------------
            \includegraphics[width=0.18\textwidth]{images/reconstruction/mtf__r4_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-inversion__r4_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-solver__r4_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_r5_v2.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/ddim_bird_round3.jpg} \\
            
            % 第四行----------------------
           \includegraphics[width=0.18\textwidth]{images/reconstruction/mtflow_r8.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-inversion_bird_r8.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/rf-solver_bird_r8.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/fireflow_bird_r8.jpg} &
            \includegraphics[width=0.18\textwidth]{images/reconstruction/ddim_bird_round8.jpg} 
        \end{tabular}
    \end{minipage} \\
    \end{tabular}

    \captionsetup{skip=0pt}
    \caption{\textbf{Multi-turn Reconstruction Results.} This figure compares image reconstructions using our method and baseline methods across 1, 2, 4, and 8 reconstruction iterations. Our method effectively preserves color, background, structure, and semantic consistency across multiple reconstruction rounds, outperforming the baseline methods.}
    \label{fig:multi_turn_reconstrution_double}

\end{figure*}

==> figures/multi_turn_reconstruction.tex <==
\begin{figure}[htbp]
    \centering
    \begin{tabular}{ccccc} % 定义 4 列
source & Round 1 & Round 2 & Round 3 \\% 
    % 第二行：第一行图片
    \begin{tikzpicture}
    \node[draw=OliveGreen, line width=2pt, inner sep=0pt] {
    \includegraphics[width=0.08\textwidth]{images/reconstruction/vermeer.jpg}}; 
    \end{tikzpicture}&
    \includegraphics[width=0.08\textwidth]{images/reconstruction/img_18.jpg} &
    \includegraphics[width=0.08\textwidth]{images/reconstruction/fireflow_img_0_vermeer_15steps_guidance2_2_inject-step0_r2.jpg} &
    \includegraphics[width=0.08\textwidth]{images/reconstruction/fireflow_img_0_vermeer_15steps_guidance2_2_2inject-step0_r3.jpg} & 
    \scalebox{0.9}{\raisebox{1.4cm}{\rotatebox{270}{FireFlow}}} \\
    
    % 第三行：第二行图片
    \begin{tikzpicture}
    \node[draw=OliveGreen, line width=2pt, inner sep=0pt] {
    \includegraphics[width=0.08\textwidth]{images/reconstruction/vermeer.jpg}}; 
    \end{tikzpicture}&
    \includegraphics[width=0.08\textwidth]{images/reconstruction/rf_solvevermeer_17_steps.png} &
    \includegraphics[width=0.08\textwidth]{images/reconstruction/rf_solve_img_0_vermeer_20steps_guidance2_2inject-step0_r2.jpg} &
    \includegraphics[width=0.08\textwidth]{images/reconstruction/rf_solver_img_0_vermeer_20steps_guidance2_2_2inject-step0_r3.jpg} &
    \scalebox{0.9}{\raisebox{1.5cm}{\rotatebox{270}{RF-Solver}}}\\
    
    % 第四行：第三行图片
      \begin{tikzpicture}
    \node[draw=OliveGreen, line width=2pt, inner sep=0pt] {
    \includegraphics[width=0.08\textwidth]{images/reconstruction/vermeer.jpg}}; 
    \end{tikzpicture}&
    \includegraphics[width=0.08\textwidth]{images/reconstruction/rf_inversion_r1.png} &
    \includegraphics[width=0.08\textwidth]{images/reconstruction/rf_inversion_r2.png} &
    \includegraphics[width=0.08\textwidth]{images/reconstruction/rf_inversion_r3.png} &
    \scalebox{0.9}{\raisebox{1.6cm}{\rotatebox{270}{RF-Inversion}}}\\
    
    % 第五行：第四行图片
    \begin{tikzpicture}
    \node[draw=OliveGreen, line width=2pt, inner sep=0pt] {
    \includegraphics[width=0.08\textwidth]{images/reconstruction/vermeer.jpg}}; 
    \end{tikzpicture} &

    \begin{tikzpicture}
    \node[draw=BrickRed, line width=2pt, inner sep=0pt] {
    \includegraphics[width=0.08\textwidth]{images/reconstruction/mtf_r1.png}};
    \end{tikzpicture} &

    \begin{tikzpicture}
    \node[draw=BrickRed, line width=2pt, inner sep=0pt] {
    \includegraphics[width=0.08\textwidth]{images/reconstruction/mtf_r2.png}};
    \end{tikzpicture}
    &
    \begin{tikzpicture}
    \node[draw=BrickRed, line width=2pt, inner sep=0pt] {
    \includegraphics[width=0.08\textwidth]{images/reconstruction/mtf_r3.png}}; 
    \end{tikzpicture}
    &
    \scalebox{0.9}{\raisebox{1.2cm}{\rotatebox{270}{Ours}}}
    \end{tabular}
    
    % 添加整体图标题
    \caption{Multi-round Reconstruction}
    \label{fig:multi_turn_reconstruction}
\end{figure}

==> figures/subfigure_template.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> figures/tease.tex <==
\begin{figure*}[t]
\centering
    \captionsetup[subfigure]{labelformat=empty, justification=centering, singlelinecheck=false}
    \setlength{\tabcolsep}{3pt}
    
    % 自定义一个带有箭头和文字的分隔符
    \newcommand{\arrowwithtext}[2][OliveGreen, very thick]{
    \begin{tikzpicture}[baseline=-0.5ex]
        % 绘制箭头，设置颜色、线宽和箭头样式
        \draw[->, line width=1pt, draw=#1, >=Latex] (-5,0) -- (6,0); 
        % 添加文字说明
        \node[below=2pt, align=center, text=#1] at (0,0) {#2}; 
    \end{tikzpicture}%
}

    \begin{tabular}{cccccc}
        \begin{subfigure}[t]{0.15\textwidth}
            \includegraphics[width=\linewidth]{images/tease/000000000001.jpg}
            \caption{source}
            \label{fig:sub1a}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}
            \includegraphics[width=\linewidth]{images/tease/square_cake.jpg}
            \caption{\sout{round} $\rightarrow$ \textcolor{BrickRed}{\textit{square}}}
            \label{fig:sub1b}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}          
            \includegraphics[width=\linewidth]{images/tease/square_cake_frosting.jpg}
            \caption{$+$~\textcolor{BrickRed}{\textit{frosting}}}
            \label{fig:sub1c}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}      
            \includegraphics[width=\linewidth]{images/tease/square cake with blue frosting.jpg}
            \caption{\textcolor{BrickRed}{\textit{[blue]}} frosting}
            \label{fig:sub1d}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth} 
            \includegraphics[width=\linewidth]{images/tease/square_cake_strawberry.jpg}
            \caption{$+$~\textcolor{BrickRed}{\textit{strawberry}}}
            \label{fig:sub1e}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}
            \includegraphics[width=\linewidth]{images/tease/a square cake with blue frosting and a car on center top of the cake_multi_turn_rf_inversionimg_0_test_pie_15steps_guidance3.5_inject-step0.jpg}
            \caption{\sout{strawberry} $\rightarrow$ \textcolor{BrickRed}{\textit{car}}}
            \label{fig:sub1f}
        \end{subfigure} \\

        % 使用自定义命令替换 \hline 并增加行间距
        \multicolumn{6}{c}{\vspace{1em}\arrowwithtext
        {\textit{
        Each editing round builds upon the results of the preceding round}}} \\

        \begin{subfigure}[t]{0.15\textwidth}
        \setlength{\fboxsep}{0pt}
            \fcolorbox{gray}{white}{\includegraphics[width=\linewidth]{images/tease/112000000003.jpg}}
            \caption{source}
            \label{fig:sub2a}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth} 
        \setlength{\fboxsep}{0pt}
            \fcolorbox{gray}{white}{\includegraphics[width=\linewidth]{images/tease/a girl with black hair and a white shirt is holding a coffee_img_0.jpg}}
            \caption{\sout{phone} $\rightarrow$ \textcolor{BrickRed}{\textit{coffee}}}
            \label{fig:sub2b}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}        \setlength{\fboxsep}{0pt}
            \fcolorbox{gray}{white}           {\includegraphics[width=\linewidth]{images/tease/a girl with black hair and a white shirt is holding a coffee and a book_img_0.jpg}}
            \caption{+ \textcolor{BrickRed}{\textit{book}}}
            \label{fig:sub2c}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}
        \setlength{\fboxsep}{0pt}
            \fcolorbox{gray}{white}{
            \includegraphics[width=\linewidth]{images/tease/a girl with black hair and a red shirt is holding a coffee and a book_img_0.jpg}}
            \caption{\sout{white} \textit{\textcolor{BrickRed}{[red]}} skirt}
            \label{fig:sub2d}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}           \setlength{\fboxsep}{0pt}
            \fcolorbox{gray}{white}
            {\includegraphics[width=\linewidth]{images/tease/a girl with black hair and a red shirt is holding a coffee and a book, carrying schoolbag on the back.jpg}}
            \caption{+ \textcolor{BrickRed}{\textit{schoolbag}}}
            \label{fig:sub2e}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\textwidth}
        \setlength{\fboxsep}{0pt}
            \fcolorbox{gray}{white}
           {\includegraphics[width=\linewidth]{images/tease/a girl with black hair and is holding a coffee and a bunch of flower, carrying schoolbag on the back.jpg}}
            \caption{\sout{book}$\rightarrow$\textcolor{BrickRed}{\textit{a bunch of flower}}}
            \label{fig:sub2f}
        \end{subfigure}
    \end{tabular}
    \caption{Workflow of multi-turn image editing. Allowing users gradually refine their requirements.}
    \label{fig:tease}
\end{figure*}

